Array Synthesis in Terms of Characteristic Modes and Generalized Scattering Matrices

The synthesis of antenna arrays in presence of mutual coupling using generalized scattering matrices in terms of characteristic modes is proposed. For the synthesis, the array is built of synthetic elements that are described by their modal scattering and radiation behavior. In particular, the question of how to describe the degrees of freedom of such elements is addressed. The eigenvalues of the characteristic modes of the element geometry and the modal radiation behavior of the antenna are thereby selected as degrees of freedom for the model of the synthetic elements. Using this model and a modal coupling matrix, an approach to optimize the modal configuration of the elements within an array is proposed. Finally, a close to reality example shows how the proposed theory can be used to enhance the cross-polarization rejection of a circularly polarized patch antenna array with a fixed beam.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> images/higher_order_coupling_mode_1.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.419; green,203.337; blue,50.337},draw={rgb,255: red,253.419; green,203.337; blue,50.337}](-0.070637, -1.2) -- (0.070637, -1.2) -- (0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,160.5735; green,200.4045; blue,64.2855},draw={rgb,255: red,160.5735; green,200.4045; blue,64.2855}](-0.070637, 0.15) -- (0.070637, 0.3) -- (-0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.070637, -0.15) -- (0.070637, 0) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.5995; green,249.441; blue,22.236},draw={rgb,255: red,248.5995; green,249.441; blue,22.236}](-0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.070637, -0.9) -- (0.070637, -0.9) -- (0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.070637, -1.05) -- (0.070637, -1.05) -- (0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.5995; green,249.441; blue,22.236},draw={rgb,255: red,248.5995; green,249.441; blue,22.236}](0.070637, -0.75) -- (0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.070637, -0.15) -- (0.070637, -0.15) -- (0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,211.1655; green,190.7655; blue,39.168},draw={rgb,255: red,211.1655; green,190.7655; blue,39.168}](-0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,160.5735; green,200.4045; blue,64.2855},draw={rgb,255: red,160.5735; green,200.4045; blue,64.2855}](0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.070637, -0.9) -- (0.070637, -0.75) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.7225; green,202.7505; blue,136.68},draw={rgb,255: red,68.7225; green,202.7505; blue,136.68}](-0.070637, -1.35) -- (-0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.070637, -1.5) -- (0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,228.5565; blue,38.4285},draw={rgb,255: red,244.8255; green,228.5565; blue,38.4285}](-0.070637, -1.2) -- (0.070637, -1.05) -- (-0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.5395; green,239.1645; blue,32.1555},draw={rgb,255: red,245.5395; green,239.1645; blue,32.1555}](0.070637, -0.6) -- (-0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.070637, -1.05) -- (0.070637, -0.9) -- (-0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.070637, 0.15) -- (0.070637, 0.15) -- (0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,211.1655; green,190.7655; blue,39.168},draw={rgb,255: red,211.1655; green,190.7655; blue,39.168}](-0.070637, 0.3) -- (0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.070637, 0.75) -- (0.070637, 0.9) -- (-0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.070637, 0.6) -- (-0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,228.5565; blue,38.4285},draw={rgb,255: red,244.8255; green,228.5565; blue,38.4285}](0.070637, 1.05) -- (0.070637, 1.2) -- (-0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.070637, 1.35) -- (-0.070637, 1.35) -- (-0.070637, 1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.7225; green,202.7505; blue,136.68},draw={rgb,255: red,68.7225; green,202.7505; blue,136.68}](0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.5395; green,239.1645; blue,32.1555},draw={rgb,255: red,245.5395; green,239.1645; blue,32.1555}](0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.070637, 0.45) -- (0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](-0.070637, 0.45) -- (-0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.070637, 0.9) -- (-0.070637, 0.75) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.070637, 1.2) -- (0.070637, 1.2) -- (0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.419; green,203.337; blue,50.337},draw={rgb,255: red,253.419; green,203.337; blue,50.337}](-0.070637, 1.2) -- (-0.070637, 1.05) -- (0.070637, 1.2) -- cycle;


==> images/higher_order_coupling_mode_2.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.070637, -1.2) -- (0.070637, -1.2) -- (0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.2535; green,242.097; blue,29.784},draw={rgb,255: red,246.2535; green,242.097; blue,29.784}](-0.070637, 0.15) -- (0.070637, 0.3) -- (-0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.070637, -0.15) -- (0.070637, 0) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](-0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.070637, -0.9) -- (0.070637, -0.9) -- (0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.070637, -1.05) -- (0.070637, -1.05) -- (0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](0.070637, -0.75) -- (0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.5995; green,249.441; blue,22.236},draw={rgb,255: red,248.5995; green,249.441; blue,22.236}](-0.070637, -0.15) -- (0.070637, -0.15) -- (0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.5395; green,239.1645; blue,32.1555},draw={rgb,255: red,245.5395; green,239.1645; blue,32.1555}](-0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.2535; green,242.097; blue,29.784},draw={rgb,255: red,246.2535; green,242.097; blue,29.784}](0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,234.192; green,186.354; blue,48.195},draw={rgb,255: red,234.192; green,186.354; blue,48.195}](-0.070637, -0.9) -- (0.070637, -0.75) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.070637, -1.35) -- (-0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.070637, -1.5) -- (0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.070637, -1.2) -- (0.070637, -1.05) -- (-0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.070637, -0.6) -- (-0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.070637, -1.05) -- (0.070637, -0.9) -- (-0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.070637, 0.15) -- (0.070637, 0.15) -- (0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.5395; green,239.1645; blue,32.1555},draw={rgb,255: red,245.5395; green,239.1645; blue,32.1555}](-0.070637, 0.3) -- (0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.5995; green,249.441; blue,22.236},draw={rgb,255: red,248.5995; green,249.441; blue,22.236}](-0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.070637, 0.75) -- (0.070637, 0.9) -- (-0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.070637, 0.6) -- (-0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.070637, 1.05) -- (0.070637, 1.2) -- (-0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.070637, 1.35) -- (-0.070637, 1.35) -- (-0.070637, 1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.070637, 0.45) -- (0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.070637, 0.45) -- (-0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,234.192; green,186.354; blue,48.195},draw={rgb,255: red,234.192; green,186.354; blue,48.195}](0.070637, 0.9) -- (-0.070637, 0.75) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.070637, 1.2) -- (0.070637, 1.2) -- (0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.070637, 1.2) -- (-0.070637, 1.05) -- (0.070637, 1.2) -- cycle;


==> images/higher_order_coupling_mode_3.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.070637, -1.2) -- (0.070637, -1.2) -- (0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](-0.070637, 0.15) -- (0.070637, 0.3) -- (-0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.070637, -0.15) -- (0.070637, 0) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.070637, -0.9) -- (0.070637, -0.9) -- (0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.070637, -1.05) -- (0.070637, -1.05) -- (0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.070637, -0.75) -- (0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.070637, -0.15) -- (0.070637, -0.15) -- (0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,190.179; blue,59.9505},draw={rgb,255: red,254.133; green,190.179; blue,59.9505}](-0.070637, -0.45) -- (0.070637, -0.3) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.070637, -0.9) -- (0.070637, -0.75) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.070637, -1.2) -- (-0.070637, -1.35) -- (0.070637, -1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](-0.070637, -1.35) -- (-0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.070637, -1.5) -- (0.070637, -1.5) -- (0.070637, -1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.070637, -1.2) -- (0.070637, -1.05) -- (-0.070637, -1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.070637, -0.6) -- (-0.070637, -0.6) -- (-0.070637, -0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.070637, -0.6) -- (0.070637, -0.45) -- (-0.070637, -0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.070637, -0.3) -- (0.070637, -0.15) -- (-0.070637, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.623; green,188.8785; blue,61.047},draw={rgb,255: red,253.623; green,188.8785; blue,61.047}](-0.070637, -1.05) -- (0.070637, -0.9) -- (-0.070637, -0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.070637, 0.15) -- (0.070637, 0.15) -- (0.070637, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,190.179; blue,59.9505},draw={rgb,255: red,254.133; green,190.179; blue,59.9505}](-0.070637, 0.3) -- (0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.070637, 0) -- (0.070637, 0.15) -- (-0.070637, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.070637, 0.75) -- (0.070637, 0.9) -- (-0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.070637, 0.6) -- (-0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.070637, 1.05) -- (0.070637, 1.2) -- (-0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.070637, 1.35) -- (-0.070637, 1.35) -- (-0.070637, 1.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.070637, 1.35) -- (0.070637, 1.5) -- (-0.070637, 1.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.070637, 0.75) -- (-0.070637, 0.6) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.070637, 0.45) -- (0.070637, 0.45) -- (0.070637, 0.6) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](-0.070637, 0.45) -- (-0.070637, 0.3) -- (0.070637, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.070637, 0.9) -- (-0.070637, 0.75) -- (0.070637, 0.75) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.623; green,188.8785; blue,61.047},draw={rgb,255: red,253.623; green,188.8785; blue,61.047}](0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 0.9) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.070637, 1.05) -- (-0.070637, 0.9) -- (0.070637, 1.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.070637, 1.2) -- (0.070637, 1.2) -- (0.070637, 1.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.070637, 1.2) -- (-0.070637, 1.05) -- (0.070637, 1.2) -- cycle;


==> images/patch_mode_1.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_mode_2.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_mode_3.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.0675; green,207.978; blue,47.8125},draw={rgb,255: red,252.0675; green,207.978; blue,47.8125}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,231.8715; green,186.6855; blue,46.2825},draw={rgb,255: red,231.8715; green,186.6855; blue,46.2825}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2095; green,195.9165; blue,55.6155},draw={rgb,255: red,254.2095; green,195.9165; blue,55.6155}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.339; green,214.302; blue,44.8035},draw={rgb,255: red,249.339; green,214.302; blue,44.8035}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.1005; green,222.258; blue,41.004},draw={rgb,255: red,246.1005; green,222.258; blue,41.004}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,193.086; blue,175.4655},draw={rgb,255: red,34.527; green,193.086; blue,175.4655}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,99.858; blue,252.756},draw={rgb,255: red,68.6205; green,99.858; blue,252.756}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_mode_4.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,203.082; blue,134.283},draw={rgb,255: red,71.6295; green,203.082; blue,134.283}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.971; green,186.915; blue,62.373},draw={rgb,255: red,250.971; green,186.915; blue,62.373}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.339; green,136.3995; blue,245.8455},draw={rgb,255: red,45.339; green,136.3995; blue,245.8455}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.871; green,240.6435; blue,31.008},draw={rgb,255: red,245.871; green,240.6435; blue,31.008}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.6995; green,201.8325; blue,51.306},draw={rgb,255: red,253.6995; green,201.8325; blue,51.306}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.115; green,247.962; blue,23.919},draw={rgb,255: red,248.115; green,247.962; blue,23.919}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,227.001; blue,39.066},draw={rgb,255: red,245.004; green,227.001; blue,39.066}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.0765; green,198.5685; blue,156.723},draw={rgb,255: red,51.0765; green,198.5685; blue,156.723}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.992; green,89.9895; blue,248.9565},draw={rgb,255: red,70.992; green,89.9895; blue,248.9565}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.904; green,158.763; blue,229.449},draw={rgb,255: red,35.904; green,158.763; blue,229.449}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.6125; green,154.0965; blue,232.3815},draw={rgb,255: red,37.6125; green,154.0965; blue,232.3815}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,90.474; green,204.408; blue,119.0595},draw={rgb,255: red,90.474; green,204.408; blue,119.0595}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.8745; green,196.3245; blue,164.577},draw={rgb,255: red,45.8745; green,196.3245; blue,164.577}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_mode_5.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.698; green,230.0865; blue,37.74},draw={rgb,255: red,244.698; green,230.0865; blue,37.74}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.397; green,186.8385; blue,194.3865},draw={rgb,255: red,2.397; green,186.8385; blue,194.3865}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.5555; green,199.104; blue,154.6575},draw={rgb,255: red,52.5555; green,199.104; blue,154.6575}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,51.153; green,122.4765; blue,252.603},draw={rgb,255: red,51.153; green,122.4765; blue,252.603}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,242.8365; green,185.742; blue,57.0435},draw={rgb,255: red,242.8365; green,185.742; blue,57.0435}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.7925; green,211.14; blue,46.3335},draw={rgb,255: red,250.7925; green,211.14; blue,46.3335}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.0695; green,185.946; blue,60.5115},draw={rgb,255: red,247.0695; green,185.946; blue,60.5115}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.7525; green,141.627; blue,241.5615},draw={rgb,255: red,44.7525; green,141.627; blue,241.5615}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.926; green,192.576; blue,177.225},draw={rgb,255: red,31.926; green,192.576; blue,177.225}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.5815; green,151.725; blue,234.141},draw={rgb,255: red,38.5815; green,151.725; blue,234.141}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,80.325; blue,242.862},draw={rgb,255: red,71.7315; green,80.325; blue,242.862}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,92.769; blue,250.3335},draw={rgb,255: red,70.533; green,92.769; blue,250.3335}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.451; green,70.482; blue,234.702},draw={rgb,255: red,71.451; green,70.482; blue,234.702}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,62.322; green,39.117; blue,171.564},draw={rgb,255: red,62.322; green,39.117; blue,171.564}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.737; green,63.4695; blue,227.154},draw={rgb,255: red,70.737; green,63.4695; blue,227.154}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,52.683; green,120.9465; blue,253.113},draw={rgb,255: red,52.683; green,120.9465; blue,253.113}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.5895; green,56.8905; blue,217.464},draw={rgb,255: red,69.5895; green,56.8905; blue,217.464}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.0995; green,59.415; blue,221.646},draw={rgb,255: red,70.0995; green,59.415; blue,221.646}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.147; green,47.277; blue,194.055},draw={rgb,255: red,66.147; green,47.277; blue,194.055}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_mode_6.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,219.3; green,189.0315; blue,40.4685},draw={rgb,255: red,219.3; green,189.0315; blue,40.4685}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,167.4585; green,199.359; blue,59.3895},draw={rgb,255: red,167.4585; green,199.359; blue,59.3895}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.27; green,150.501; blue,235.059},draw={rgb,255: red,39.27; green,150.501; blue,235.059}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,113.8065; green,204.612; blue,99.552},draw={rgb,255: red,113.8065; green,204.612; blue,99.552}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,132.2685; green,203.541; blue,86.037},draw={rgb,255: red,132.2685; green,203.541; blue,86.037}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,84.1755; green,204.051; blue,124.338},draw={rgb,255: red,84.1755; green,204.051; blue,124.338}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.031; green,198.849; blue,53.4225},draw={rgb,255: red,254.031; green,198.849; blue,53.4225}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,74.6895; green,203.3625; blue,131.835},draw={rgb,255: red,74.6895; green,203.3625; blue,131.835}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,157.1055; green,200.889; blue,66.861},draw={rgb,255: red,157.1055; green,200.889; blue,66.861}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,174.2415; green,198.2115; blue,54.9525},draw={rgb,255: red,174.2415; green,198.2115; blue,54.9525}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,193.545; green,194.5395; blue,43.7835},draw={rgb,255: red,193.545; green,194.5395; blue,43.7835}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.135; green,186.252; blue,61.659},draw={rgb,255: red,249.135; green,186.252; blue,61.659}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.146; green,245.0295; blue,27.0555},draw={rgb,255: red,247.146; green,245.0295; blue,27.0555}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.687; green,243.576; blue,28.458},draw={rgb,255: red,246.687; green,243.576; blue,28.458}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,187.272; green,195.8145; blue,47.226},draw={rgb,255: red,187.272; green,195.8145; blue,47.226}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,240.72; green,185.7675; blue,54.8505},draw={rgb,255: red,240.72; green,185.7675; blue,54.8505}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,190.434; green,195.177; blue,45.441},draw={rgb,255: red,190.434; green,195.177; blue,45.441}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.789; green,195.228; blue,168.2745},draw={rgb,255: red,42.789; green,195.228; blue,168.2745}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,77.826; green,203.6175; blue,129.387},draw={rgb,255: red,77.826; green,203.6175; blue,129.387}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,170.8755; green,198.798; blue,57.0945},draw={rgb,255: red,170.8755; green,198.798; blue,57.0945}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,128.622; green,203.8215; blue,88.74},draw={rgb,255: red,128.622; green,203.8215; blue,88.74}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.133; green,197.37; blue,54.519},draw={rgb,255: red,254.133; green,197.37; blue,54.519}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,110.211; green,204.714; blue,102.3315},draw={rgb,255: red,110.211; green,204.714; blue,102.3315}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,80.988; green,203.847; blue,126.8625},draw={rgb,255: red,80.988; green,203.847; blue,126.8625}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.5205; green,202.011; blue,141.423},draw={rgb,255: red,63.5205; green,202.011; blue,141.423}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.2255; green,201.5775; blue,143.718},draw={rgb,255: red,61.2255; green,201.5775; blue,143.718}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.222; green,200.6595; blue,148.2315},draw={rgb,255: red,57.222; green,200.6595; blue,148.2315}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,96.7725; green,204.663; blue,113.577},draw={rgb,255: red,96.7725; green,204.663; blue,113.577}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,153.612; green,201.348; blue,69.513},draw={rgb,255: red,153.612; green,201.348; blue,69.513}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,121.2015; green,204.2805; blue,94.1205},draw={rgb,255: red,121.2015; green,204.2805; blue,94.1205}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,177.5565; green,197.625; blue,52.9125},draw={rgb,255: red,177.5565; green,197.625; blue,52.9125}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,213.9195; green,190.1535; blue,39.423},draw={rgb,255: red,213.9195; green,190.1535; blue,39.423}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,99.9855; green,204.7395; blue,110.772},draw={rgb,255: red,99.9855; green,204.7395; blue,110.772}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,196.605; green,193.902; blue,42.279},draw={rgb,255: red,196.605; green,193.902; blue,42.279}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,216.6225; green,189.5925; blue,39.882},draw={rgb,255: red,216.6225; green,189.5925; blue,39.882}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,224.502; green,187.986; blue,42.075},draw={rgb,255: red,224.502; green,187.986; blue,42.075}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,143.0295; green,202.5465; blue,77.775},draw={rgb,255: red,143.0295; green,202.5465; blue,77.775}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,202.5975; green,192.627; blue,40.035},draw={rgb,255: red,202.5975; green,192.627; blue,40.035}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,150.093; green,201.7815; blue,72.2415},draw={rgb,255: red,150.093; green,201.7815; blue,72.2415}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_port_1.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_port_2.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.993; green,145.4775; blue,238.6035},draw={rgb,255: red,42.993; green,145.4775; blue,238.6035}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.0985; green,128.265; blue,250.3845},draw={rgb,255: red,47.0985; green,128.265; blue,250.3845}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,4.131; green,187.476; blue,192.729},draw={rgb,255: red,4.131; green,187.476; blue,192.729}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,37.2555; green,155.2695; blue,231.54},draw={rgb,255: red,37.2555; green,155.2695; blue,231.54}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.724; green,171.105; blue,221.7225},draw={rgb,255: red,26.724; green,171.105; blue,221.7225}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.376; green,167.892; blue,224.502},draw={rgb,255: red,29.376; green,167.892; blue,224.502}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.982; green,140.352; blue,242.658},draw={rgb,255: red,44.982; green,140.352; blue,242.658}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,221.9265; green,188.496; blue,41.1825},draw={rgb,255: red,221.9265; green,188.496; blue,41.1825}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,208.386; green,191.3775; blue,39.1425},draw={rgb,255: red,208.386; green,191.3775; blue,39.1425}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.0615; green,110.1345; blue,254.5665},draw={rgb,255: red,63.0615; green,110.1345; blue,254.5665}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.1705; green,88.6125; blue,248.1915},draw={rgb,255: red,71.1705; green,88.6125; blue,248.1915}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,78.9225; blue,241.8165},draw={rgb,255: red,71.757; green,78.9225; blue,241.8165}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,29.0955; green,192.0405; blue,178.9845},draw={rgb,255: red,29.0955; green,192.0405; blue,178.9845}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.055; green,148.0275; blue,236.8695},draw={rgb,255: red,41.055; green,148.0275; blue,236.8695}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.3955; green,195.789; blue,166.4385},draw={rgb,255: red,44.3955; green,195.789; blue,166.4385}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,199.6395; green,193.2645; blue,41.004},draw={rgb,255: red,199.6395; green,193.2645; blue,41.004}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,135.8895; green,203.235; blue,83.3085},draw={rgb,255: red,135.8895; green,203.235; blue,83.3085}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,254.2605; green,194.463; blue,56.712},draw={rgb,255: red,254.2605; green,194.463; blue,56.712}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,41.0295; green,194.6925; blue,170.1105},draw={rgb,255: red,41.0295; green,194.6925; blue,170.1105}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.004; green,236.181; blue,34.272},draw={rgb,255: red,245.004; green,236.181; blue,34.272}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,24.582; green,173.1195; blue,219.5295},draw={rgb,255: red,24.582; green,173.1195; blue,219.5295}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.924; green,193.6215; blue,173.706},draw={rgb,255: red,36.924; green,193.6215; blue,173.706}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,12.852; green,189.2865; blue,187.6545},draw={rgb,255: red,12.852; green,189.2865; blue,187.6545}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.2845; green,225.42; blue,39.7035},draw={rgb,255: red,245.2845; green,225.42; blue,39.7035}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,55.539; green,200.1495; blue,150.4245},draw={rgb,255: red,55.539; green,200.1495; blue,150.4245}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.8255; green,234.6765; blue,35.241},draw={rgb,255: red,244.8255; green,234.6765; blue,35.241}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,252.603; green,206.4225; blue,48.603},draw={rgb,255: red,252.603; green,206.4225; blue,48.603}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,248.574; green,215.9085; blue,44.013},draw={rgb,255: red,248.574; green,215.9085; blue,44.013}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,59.109; green,201.1185; blue,145.9875},draw={rgb,255: red,59.109; green,201.1185; blue,145.9875}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,87.312; green,204.2295; blue,121.737},draw={rgb,255: red,87.312; green,204.2295; blue,121.737}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.667; green,223.839; blue,40.341},draw={rgb,255: red,245.667; green,223.839; blue,40.341}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.827; green,198.0075; blue,158.7375},draw={rgb,255: red,49.827; green,198.0075; blue,158.7375}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,6.4515; green,188.088; blue,191.046},draw={rgb,255: red,6.4515; green,188.088; blue,191.046}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,9.4095; green,188.7; blue,189.363},draw={rgb,255: red,9.4095; green,188.7; blue,189.363}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,2.3205; green,182.6565; blue,204.0765},draw={rgb,255: red,2.3205; green,182.6565; blue,204.0765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,39.066; green,194.157; blue,171.8955},draw={rgb,255: red,39.066; green,194.157; blue,171.8955}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,186.1755; blue,196.044},draw={rgb,255: red,1.173; green,186.1755; blue,196.044}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,1.173; green,183.396; blue,202.4955},draw={rgb,255: red,1.173; green,183.396; blue,202.4955}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,20.1195; green,176.001; blue,215.781},draw={rgb,255: red,20.1195; green,176.001; blue,215.781}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.2295; green,184.824; blue,199.2825},draw={rgb,255: red,0.2295; green,184.824; blue,199.2825}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.269; green,189.873; blue,185.946},draw={rgb,255: red,16.269; green,189.873; blue,185.946}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,8.364; green,180.3105; blue,208.6665},draw={rgb,255: red,8.364; green,180.3105; blue,208.6665}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.1835; green,108.6555; blue,254.337},draw={rgb,255: red,64.1835; green,108.6555; blue,254.337}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.227; green,94.1715; blue,250.92},draw={rgb,255: red,70.227; green,94.1715; blue,250.92}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.87; green,58.14; blue,219.606},draw={rgb,255: red,69.87; green,58.14; blue,219.606}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.6205; green,53.397; blue,210.3495},draw={rgb,255: red,68.6205; green,53.397; blue,210.3495}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4985; green,102.765; blue,253.3425},draw={rgb,255: red,67.4985; green,102.765; blue,253.3425}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,63.8265; green,42.024; blue,180.3105},draw={rgb,255: red,63.8265; green,42.024; blue,180.3105}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,69.054; blue,233.325},draw={rgb,255: red,71.349; green,69.054; blue,233.325}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.238; green,52.326; blue,207.774},draw={rgb,255: red,68.238; green,52.326; blue,207.774}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.8955; green,95.574; blue,251.481},draw={rgb,255: red,69.8955; green,95.574; blue,251.481}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,33.6855; green,162.2565; blue,227.766},draw={rgb,255: red,33.6855; green,162.2565; blue,227.766}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,38.046; green,152.9235; blue,233.2485},draw={rgb,255: red,38.046; green,152.9235; blue,233.2485}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.8355; green,104.244; blue,253.623},draw={rgb,255: red,66.8355; green,104.244; blue,253.623}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,48.5265; green,125.4345; blue,251.6085},draw={rgb,255: red,48.5265; green,125.4345; blue,251.6085}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.7315; green,76.1175; blue,239.6235},draw={rgb,255: red,71.7315; green,76.1175; blue,239.6235}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.084; green,139.026; blue,243.78},draw={rgb,255: red,45.084; green,139.026; blue,243.78}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,11.0415; green,179.4945; blue,210.171},draw={rgb,255: red,11.0415; green,179.4945; blue,210.171}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.4395; green,157.59; blue,230.061},draw={rgb,255: red,36.4395; green,157.59; blue,230.061}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,16.014; green,177.786; blue,213.0525},draw={rgb,255: red,16.014; green,177.786; blue,213.0525}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,34.527; green,161.0835; blue,228.3015},draw={rgb,255: red,34.527; green,161.0835; blue,228.3015}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,36.873; green,156.4425; blue,230.775},draw={rgb,255: red,36.873; green,156.4425; blue,230.775}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,30.2175; green,166.7955; blue,225.267},draw={rgb,255: red,30.2175; green,166.7955; blue,225.267}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,13.6425; green,178.653; blue,211.6245},draw={rgb,255: red,13.6425; green,178.653; blue,211.6245}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,18.1815; green,176.919; blue,214.4295},draw={rgb,255: red,18.1815; green,176.919; blue,214.4295}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.105; green,98.43; blue,252.399},draw={rgb,255: red,69.105; green,98.43; blue,252.399}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,35.2665; green,159.936; blue,228.8625},draw={rgb,255: red,35.2665; green,159.936; blue,228.8625}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.2115; green,137.7255; blue,244.851},draw={rgb,255: red,45.2115; green,137.7255; blue,244.851}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,44.37; green,142.9275; blue,240.516},draw={rgb,255: red,44.37; green,142.9275; blue,240.516}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.6905; green,129.642; blue,249.7215},draw={rgb,255: red,46.6905; green,129.642; blue,249.7215}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,32.844; green,163.404; blue,227.205},draw={rgb,255: red,32.844; green,163.404; blue,227.205}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,31.9515; green,164.5515; blue,226.6185},draw={rgb,255: red,31.9515; green,164.5515; blue,226.6185}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_port_3.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/patch_port_4.tex <==
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0) -- (0.35, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.071429, 0.071429) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3949, 0.094156) -- (0.2949, 0.094156) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0.076125, 0.031135) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.15, 0.040644) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, 0.031135) -- (0.1, 0) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, 0.13808) -- (0.17613, 0.031135) -- (0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.1) -- (0.46887, 0.12613) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2949, 0.094156) -- (0.3949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.46887, 0.12613) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.5, 0.3) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35017, 0.29269) -- (0.40584, 0.2449) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.3895, 0.2) -- (0.46887, 0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.05) -- (0.45, 0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.37613, 0.031135) -- (0.45, 0.040644) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.1) -- (0.45936, 0.1) -- (0.5, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.5, 0.1) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.12613) -- (0.45936, 0.1) -- (0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.45936, 0.1) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0.040644) -- (0.5, 0.05) -- (0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27874, 0.22126) -- (0.25354, 0.20951) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35, 0.040644) -- (0.37613, 0.031135) -- (0.3949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25354, 0.20951) -- (0.20731, 0.14983) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27613, 0.031135) -- (0.3, 0) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2949, 0.094156) -- (0.27613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0) -- (0.45, 0.040644) -- (0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35, 0) -- (0.37613, 0.031135) -- (0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0) -- (0.37613, 0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, 0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27613, 0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.27613, 0.031135) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.25, 0) -- (0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.15, 0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, 0.040644) -- (0.17613, 0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27874, 0.22126) -- (0.2949, 0.094156) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, 0.031135) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, 0.031135) -- (0.18211, 0.13808) -- (0.15, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.15, 0.040644) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.20731, 0.14983) -- (0.25, 0.040644) -- (0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.18211, 0.13808) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.10714, 0.10714) -- (0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, 0.13808) -- (0.20731, 0.14983) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, 0.13808) -- (0.25, 0.040644) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32497, 0.28094) -- (0.27874, 0.22126) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3949, 0.094156) -- (0.46887, 0.12613) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.40584, 0.2449) -- (0.32497, 0.28094) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.17857, 0.17857) -- (0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.2) -- (0.40584, 0.2449) -- (0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35017, 0.29269) -- (0.32497, 0.28094) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, 0.28571) -- (0.25, 0.25) -- (0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, 0.21429) -- (0.20731, 0.14983) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.27874, 0.22126) -- (0.25, 0.25) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.25, 0.25) -- (0.21429, 0.21429) -- (0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.32497, 0.28094) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.35017, 0.29269) -- (0.35714, 0.35714) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](0.3964, 0.35237) -- (0.39286, 0.39286) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.32143, 0.32143) -- (0.32497, 0.28094) -- (0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, 0.28571) -- (0.27874, 0.22126) -- (0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.3) -- (0.3964, 0.35237) -- (0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](0.35714, 0.35714) -- (0.35017, 0.29269) -- (0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.42857, 0.42857) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](0.39286, 0.39286) -- (0.3964, 0.35237) -- (0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.5, 0.35) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46429, 0.46429) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.4) -- (0.46887, 0.42613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, 0.46429) -- (0.42857, 0.42857) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, 0.42857) -- (0.45936, 0.4) -- (0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.46887, 0.32613) -- (0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.4) -- (0.46887, 0.32613) -- (0.5, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, 0.36412) -- (0.3964, 0.35237) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.5, 0.25) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.32613) -- (0.4216, 0.36412) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.45936, 0.2) -- (0.5, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, 0.22613) -- (0.40584, 0.2449) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.2) -- (0.46887, 0.22613) -- (0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, 0.3) -- (0.40584, 0.2449) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.25) -- (0.45936, 0.3) -- (0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.3) -- (0.46887, 0.32613) -- (0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.35) -- (0.46887, 0.32613) -- (0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.45) -- (0.46887, 0.42613) -- (0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, 0.5) -- (0.46429, 0.46429) -- (0.5, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.035714, 0.035714) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0, 0.15) -- (-0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, 0.2) -- (0, 0.25) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (-0.040644, 0.15) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.071429, 0.071429) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.13808, 0.18211) -- (-0.031135, 0.17613) -- (-0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.29269, 0.35017) -- (-0.2449, 0.40584) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.32143, 0.32143) -- (-0.29269, 0.35017) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.39286, 0.39286) -- (-0.35237, 0.3964) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.094156, 0.3949) -- (-0.040644, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, 0.28571) -- (-0.25, 0.25) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.2, 0.5) -- (-0.22613, 0.46887) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.1, 0.45936) -- (-0.094156, 0.3949) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](-0.22613, 0.46887) -- (-0.25, 0.5) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.17613) -- (-0.040644, 0.15) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.2449, 0.40584) -- (-0.28094, 0.32497) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.040644, 0.45) -- (0, 0.45) -- (0, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.05) -- (0, 0.1) -- (-0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0, 0.3) -- (-0.031135, 0.27613) -- (0, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.040644, 0.35) -- (-0.094156, 0.2949) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.040644, 0.35) -- (0, 0.3) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.2, 0.3895) -- (-0.22126, 0.27874) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](-0.031135, 0.27613) -- (0, 0.3) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.040644, 0.45) -- (-0.031135, 0.37613) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.040644, 0.35) -- (0, 0.35) -- (-0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.040644, 0.25) -- (-0.031135, 0.27613) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](-0.040644, 0.25) -- (0, 0.25) -- (-0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0, 0.2) -- (-0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.040644, 0.25) -- (-0.031135, 0.17613) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](-0.040644, 0.25) -- (-0.094156, 0.2949) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, 0.076125) -- (-0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.10714, 0.10714) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, 0.15) -- (-0.031135, 0.17613) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](-0.17857, 0.17857) -- (-0.13808, 0.18211) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.040644, 0.15) -- (-0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.13808, 0.18211) -- (-0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.22126, 0.27874) -- (-0.20951, 0.25354) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.13808, 0.18211) -- (-0.040644, 0.25) -- (-0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.13808, 0.18211) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.14983, 0.20731) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.20951, 0.25354) -- (-0.14983, 0.20731) -- (-0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, 0.28571) -- (-0.28094, 0.32497) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.32143, 0.32143) -- (-0.28094, 0.32497) -- (-0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.094156, 0.3949) -- (-0.094156, 0.2949) -- (-0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.28571, 0.28571) -- (-0.22126, 0.27874) -- (-0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.25, 0.25) -- (-0.21429, 0.21429) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.15, 0.5) -- (-0.2, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.28094, 0.32497) -- (-0.22126, 0.27874) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](-0.25, 0.25) -- (-0.20951, 0.25354) -- (-0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.21429, 0.21429) -- (-0.14983, 0.20731) -- (-0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.32613, 0.46887) -- (-0.3, 0.45936) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.2449, 0.40584) -- (-0.2, 0.3895) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](-0.36412, 0.4216) -- (-0.35237, 0.3964) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.35714, 0.35714) -- (-0.29269, 0.35017) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.4, 0.45936) -- (-0.36412, 0.4216) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.39286, 0.39286) -- (-0.35714, 0.35714) -- (-0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.4, 0.45936) -- (-0.42857, 0.42857) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](-0.4, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.42857, 0.42857) -- (-0.39286, 0.39286) -- (-0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.42613, 0.46887) -- (-0.42857, 0.42857) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](-0.42613, 0.46887) -- (-0.46429, 0.46429) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.5, 0.5) -- (-0.46429, 0.46429) -- (-0.45, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.35, 0.5) -- (-0.4, 0.5) -- (-0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.45, 0.5) -- (-0.46429, 0.46429) -- (-0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.45, 0.5) -- (-0.42613, 0.46887) -- (-0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.4, 0.45936) -- (-0.32613, 0.46887) -- (-0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, 0.4216) -- (-0.3, 0.45936) -- (-0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.35, 0.5) -- (-0.32613, 0.46887) -- (-0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, 0.46887) -- (-0.1, 0.5) -- (-0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.22613, 0.46887) -- (-0.3, 0.45936) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](-0.3, 0.5) -- (-0.3, 0.45936) -- (-0.25, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.2, 0.45936) -- (-0.22613, 0.46887) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.2, 0.5) -- (-0.25, 0.5) -- (-0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.12613, 0.46887) -- (-0.2, 0.45936) -- (-0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.12613, 0.46887) -- (-0.15, 0.5) -- (-0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35237, 0.3964) -- (-0.2449, 0.40584) -- (-0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.29269, 0.35017) -- (-0.28094, 0.32497) -- (-0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.2, 0.3895) -- (-0.094156, 0.3949) -- (-0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.2, 0.3895) -- (-0.094156, 0.2949) -- (-0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.040644, 0.45) -- (0, 0.4) -- (0, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.031135, 0.37613) -- (0, 0.35) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.12613, 0.46887) -- (-0.1, 0.45936) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.094156, 0.3949) -- (-0.031135, 0.37613) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.05, 0.5) -- (-0.1, 0.45936) -- (-0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.12613, 0.46887) -- (-0.094156, 0.3949) -- (-0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.1, 0.45936) -- (-0.05, 0.5) -- (-0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](-0.040644, 0.45) -- (0, 0.5) -- (-0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3, 0) -- (0.35, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.071429, -0.071429) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3949, -0.094156) -- (0.2949, -0.094156) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.15, 0) -- (0.2, 0) -- (0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0.076125, -0.031135) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.1, 0) -- (0.15, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.15, -0.040644) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.076125, -0.031135) -- (0.1, 0) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, -0.13808) -- (0.17613, -0.031135) -- (0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.1) -- (0.46887, -0.12613) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2949, -0.094156) -- (0.3949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.46887, -0.12613) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.5, -0.3) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35017, -0.29269) -- (0.40584, -0.2449) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.3895, -0.2) -- (0.46887, -0.12613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.05) -- (0.45, -0.040644) -- (0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.37613, -0.031135) -- (0.45, -0.040644) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.5, 0) -- (0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.1) -- (0.45936, -0.1) -- (0.5, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.5, -0.1) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.12613) -- (0.45936, -0.1) -- (0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.45936, -0.1) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, -0.040644) -- (0.5, -0.05) -- (0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27874, -0.22126) -- (0.25354, -0.20951) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35, -0.040644) -- (0.37613, -0.031135) -- (0.3949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25354, -0.20951) -- (0.20731, -0.14983) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27613, -0.031135) -- (0.3, 0) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.2949, -0.094156) -- (0.27613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0) -- (0.45, -0.040644) -- (0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35, 0) -- (0.37613, -0.031135) -- (0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4, 0) -- (0.37613, -0.031135) -- (0.35, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45, 0) -- (0.45, -0.040644) -- (0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27613, -0.031135) -- (0.25, 0) -- (0.3, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.27613, -0.031135) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.25, 0) -- (0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.2, 0) -- (0.25, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.15, -0.040644) -- (0.15, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.25, -0.040644) -- (0.17613, -0.031135) -- (0.2, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.27874, -0.22126) -- (0.2949, -0.094156) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.1, 0) -- (0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.05, 0) -- (0.076125, -0.031135) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17613, -0.031135) -- (0.18211, -0.13808) -- (0.15, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.15, -0.040644) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.20731, -0.14983) -- (0.25, -0.040644) -- (0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.18211, -0.13808) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.10714, -0.10714) -- (0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, -0.13808) -- (0.20731, -0.14983) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.18211, -0.13808) -- (0.25, -0.040644) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.32497, -0.28094) -- (0.27874, -0.22126) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.3949, -0.094156) -- (0.46887, -0.12613) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.40584, -0.2449) -- (0.32497, -0.28094) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.17857, -0.17857) -- (0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.2) -- (0.40584, -0.2449) -- (0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.35017, -0.29269) -- (0.32497, -0.28094) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, -0.28571) -- (0.25, -0.25) -- (0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.21429, -0.21429) -- (0.20731, -0.14983) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.27874, -0.22126) -- (0.25, -0.25) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.25, -0.25) -- (0.21429, -0.21429) -- (0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.32497, -0.28094) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.35017, -0.29269) -- (0.35714, -0.35714) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](0.3964, -0.35237) -- (0.39286, -0.39286) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.32143, -0.32143) -- (0.32497, -0.28094) -- (0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](0.28571, -0.28571) -- (0.27874, -0.22126) -- (0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.3) -- (0.3964, -0.35237) -- (0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](0.35714, -0.35714) -- (0.35017, -0.29269) -- (0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.42857, -0.42857) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](0.39286, -0.39286) -- (0.3964, -0.35237) -- (0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.5, -0.35) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46429, -0.46429) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.4) -- (0.46887, -0.42613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46429, -0.46429) -- (0.42857, -0.42857) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.42857, -0.42857) -- (0.45936, -0.4) -- (0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.46887, -0.32613) -- (0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.4) -- (0.46887, -0.32613) -- (0.5, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.4216, -0.36412) -- (0.3964, -0.35237) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.5, -0.25) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.32613) -- (0.4216, -0.36412) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.45936, -0.2) -- (0.5, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.46887, -0.22613) -- (0.40584, -0.2449) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.2) -- (0.46887, -0.22613) -- (0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.45936, -0.3) -- (0.40584, -0.2449) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.25) -- (0.45936, -0.3) -- (0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.3) -- (0.46887, -0.32613) -- (0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.35) -- (0.46887, -0.32613) -- (0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.45) -- (0.46887, -0.42613) -- (0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.5, -0.5) -- (0.46429, -0.46429) -- (0.5, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.35237, 0.3964) -- (0.35714, 0.35714) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.071429, 0.071429) -- (0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](0.36412, 0.4216) -- (0.35237, 0.3964) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.1, 0.5) -- (0.1, 0.45936) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.2, 0.5) -- (0.2, 0.45936) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.076125) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.2) -- (0.031135, 0.17613) -- (0, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.094156, 0.2949) -- (0.040644, 0.35) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.1) -- (0.031135, 0.076125) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](0.14983, 0.20731) -- (0.040644, 0.25) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.031135, 0.17613) -- (0.040644, 0.25) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.040644, 0.35) -- (0.094156, 0.2949) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.2, 0.3895) -- (0.094156, 0.3949) -- (0.12613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.040644, 0.45) -- (0.094156, 0.3949) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.22126, 0.27874) -- (0.2, 0.3895) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.071429, 0.071429) -- (0.031135, 0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.39286, 0.39286) -- (0.35714, 0.35714) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](0.4, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.45, 0.5) -- (0.5, 0.5) -- (0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45, 0.5) -- (0.46429, 0.46429) -- (0.42613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.4, 0.5) -- (0.4, 0.45936) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](0.42613, 0.46887) -- (0.46429, 0.46429) -- (0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.42613, 0.46887) -- (0.42857, 0.42857) -- (0.4, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.4, 0.45936) -- (0.36412, 0.4216) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.4, 0.45936) -- (0.42857, 0.42857) -- (0.36412, 0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.32613, 0.46887) -- (0.3, 0.45936) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.22613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.2449, 0.40584) -- (0.35237, 0.3964) -- (0.29269, 0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.36412, 0.4216) -- (0.42857, 0.42857) -- (0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.4, 0.45936) -- (0.32613, 0.46887) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, 0.4216) -- (0.3, 0.45936) -- (0.32613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.32613, 0.46887) -- (0.3, 0.5) -- (0.35, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.45, 0.5) -- (0.42613, 0.46887) -- (0.4, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](0.3, 0.45936) -- (0.25, 0.5) -- (0.3, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.32143, 0.32143) -- (0.29269, 0.35017) -- (0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](0.25, 0.5) -- (0.3, 0.45936) -- (0.22613, 0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.25, 0.5) -- (0.22613, 0.46887) -- (0.2, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.3, 0.45936) -- (0.35237, 0.3964) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, 0.46887) -- (0.1, 0.5) -- (0.15, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](0.12613, 0.46887) -- (0.1, 0.45936) -- (0.1, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](0.040644, 0.45) -- (0, 0.5) -- (0.05, 0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.1, 0.45936) -- (0.12613, 0.46887) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, 0.45) -- (0.040644, 0.45) -- (0, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0, 0.45) -- (0, 0.5) -- (0.040644, 0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.031135, 0.37613) -- (0.094156, 0.3949) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.2449, 0.40584) -- (0.22613, 0.46887) -- (0.3, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.040644, 0.45) -- (0.1, 0.45936) -- (0.094156, 0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.040644, 0.45) -- (0.05, 0.5) -- (0.1, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.12613, 0.46887) -- (0.2, 0.45936) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.12613, 0.46887) -- (0.15, 0.5) -- (0.2, 0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.2, 0.45936) -- (0.2449, 0.40584) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.2, 0.45936) -- (0.22613, 0.46887) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0, 0.35) -- (0.031135, 0.37613) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0, 0.4) -- (0.040644, 0.45) -- (0.031135, 0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.21429, 0.21429) -- (0.14983, 0.20731) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.040644, 0.25) -- (0.031135, 0.27613) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](0, 0.25) -- (0.031135, 0.27613) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, 0.3) -- (0, 0.35) -- (0.040644, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](0, 0.3) -- (0.040644, 0.35) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0, 0.4) -- (0.031135, 0.37613) -- (0, 0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0, 0.25) -- (0, 0.3) -- (0.031135, 0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, 0.035714) -- (0, 0) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.040644, 0.15) -- (0, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, 0.25) -- (0.040644, 0.25) -- (0, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, 0.15) -- (0.031135, 0.17613) -- (0.040644, 0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0, 0.2) -- (0.040644, 0.25) -- (0.031135, 0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, 0.076125) -- (0.035714, 0.035714) -- (0, 0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.10714, 0.10714) -- (0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, 0.15) -- (0.031135, 0.17613) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.14983, 0.20731) -- (0.13808, 0.18211) -- (0.040644, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.040644, 0.15) -- (0.13808, 0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, 0.10714) -- (0.13808, 0.18211) -- (0.14286, 0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, 0.14286) -- (0.13808, 0.18211) -- (0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.2, 0.3895) -- (0.22126, 0.27874) -- (0.094156, 0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](0.17857, 0.17857) -- (0.13808, 0.18211) -- (0.14983, 0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.29269, 0.35017) -- (0.28094, 0.32497) -- (0.2449, 0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.094156, 0.2949) -- (0.094156, 0.3949) -- (0.2, 0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](0.25, 0.25) -- (0.20951, 0.25354) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.14983, 0.20731) -- (0.094156, 0.2949) -- (0.20951, 0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.36412, 0.4216) -- (0.39286, 0.39286) -- (0.35237, 0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25, 0.25) -- (0.22126, 0.27874) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.2, 0.3895) -- (0.2449, 0.40584) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28094, 0.32497) -- (0.32143, 0.32143) -- (0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.28094, 0.32497) -- (0.29269, 0.35017) -- (0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.28571, 0.28571) -- (0.22126, 0.27874) -- (0.28094, 0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.20951, 0.25354) -- (0.094156, 0.2949) -- (0.22126, 0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.21429, 0.21429) -- (0.20951, 0.25354) -- (0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, 0.17857) -- (0.14983, 0.20731) -- (0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.40584, 0.2449) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.32143, 0.32143) -- (-0.35017, 0.29269) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, 0.22126) -- (-0.28571, 0.28571) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.5, 0.1) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.40584, 0.2449) -- (-0.35017, 0.29269) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3964, 0.35237) -- (-0.35017, 0.29269) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](-0.39286, 0.39286) -- (-0.3964, 0.35237) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, 0.094156) -- (-0.3895, 0.2) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.32497, 0.28094) -- (-0.35017, 0.29269) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3895, 0.2) -- (-0.40584, 0.2449) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.37613, 0.031135) -- (-0.3949, 0.094156) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27613, 0.031135) -- (-0.35, 0.040644) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20731, 0.14983) -- (-0.25354, 0.20951) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, 0.035714) -- (-0.076125, 0.031135) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, 0.040644) -- (-0.076125, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, 0.031135) -- (-0.15, 0.040644) -- (-0.071429, 0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, 0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2949, 0.094156) -- (-0.20731, 0.14983) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, 0.28571) -- (-0.32497, 0.28094) -- (-0.32143, 0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.21429, 0.21429) -- (-0.25354, 0.20951) -- (-0.25, 0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, 0.094156) -- (-0.46887, 0.12613) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, 0.13808) -- (-0.15, 0.040644) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.20731, 0.14983) -- (-0.21429, 0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, 0.22126) -- (-0.25, 0.25) -- (-0.25354, 0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25354, 0.20951) -- (-0.2949, 0.094156) -- (-0.27874, 0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.15) -- (-0.5, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.25) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](-0.3964, 0.35237) -- (-0.35714, 0.35714) -- (-0.35017, 0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, 0.22126) -- (-0.32497, 0.28094) -- (-0.28571, 0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27874, 0.22126) -- (-0.3895, 0.2) -- (-0.32497, 0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.5, 0.3) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.40584, 0.2449) -- (-0.45936, 0.3) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](-0.3964, 0.35237) -- (-0.39286, 0.39286) -- (-0.35714, 0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, 0.36412) -- (-0.42857, 0.42857) -- (-0.39286, 0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, 0.36412) -- (-0.46887, 0.32613) -- (-0.45936, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, 0.36412) -- (-0.45936, 0.4) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.45) -- (-0.5, 0.5) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.46887, 0.42613) -- (-0.42857, 0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.42613) -- (-0.5, 0.45) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, 0.42857) -- (-0.46887, 0.42613) -- (-0.46429, 0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.35) -- (-0.5, 0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.4) -- (-0.5, 0.45) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.4) -- (-0.5, 0.4) -- (-0.46887, 0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.46887, 0.32613) -- (-0.4216, 0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.3) -- (-0.4216, 0.36412) -- (-0.3964, 0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.46887, 0.22613) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.2) -- (-0.5, 0.25) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.46887, 0.32613) -- (-0.5, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.35) -- (-0.45936, 0.4) -- (-0.46887, 0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.45936, 0.3) -- (-0.40584, 0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.22613) -- (-0.5, 0.25) -- (-0.45936, 0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.45936, 0.2) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.5, 0.15) -- (-0.45936, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27874, 0.22126) -- (-0.2949, 0.094156) -- (-0.3895, 0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, 0.094156) -- (-0.37613, 0.031135) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27613, 0.031135) -- (-0.2949, 0.094156) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0.040644) -- (-0.3949, 0.094156) -- (-0.2949, 0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45936, 0.1) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, 0.12613) -- (-0.3949, 0.094156) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.1) -- (-0.46887, 0.12613) -- (-0.45936, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.2) -- (-0.5, 0.2) -- (-0.46887, 0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.15) -- (-0.46887, 0.12613) -- (-0.5, 0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, 0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, 0.1) -- (-0.3949, 0.094156) -- (-0.45, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, 0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0.05) -- (-0.45, 0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0) -- (-0.37613, 0.031135) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0) -- (-0.45, 0.040644) -- (-0.37613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0) -- (-0.35, 0) -- (-0.35, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17613, 0.031135) -- (-0.2, 0) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0) -- (-0.27613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0) -- (-0.35, 0.040644) -- (-0.27613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, 0.17857) -- (-0.18211, 0.13808) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.10714, 0.10714) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, 0.14286) -- (-0.18211, 0.13808) -- (-0.17857, 0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0.040644) -- (-0.20731, 0.14983) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2949, 0.094156) -- (-0.25354, 0.20951) -- (-0.20731, 0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, 0.10714) -- (-0.15, 0.040644) -- (-0.18211, 0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, 0.071429) -- (-0.15, 0.040644) -- (-0.10714, 0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, 0.031135) -- (-0.035714, 0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, 0.13808) -- (-0.17613, 0.031135) -- (-0.25, 0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0.040644) -- (-0.15, 0) -- (-0.17613, 0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, 0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, 0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.035714, -0.035714) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0, -0.15) -- (-0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, -0.2) -- (0, -0.25) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (-0.040644, -0.15) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.071429, -0.071429) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](-0.13808, -0.18211) -- (-0.031135, -0.17613) -- (-0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.29269, -0.35017) -- (-0.2449, -0.40584) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](-0.32143, -0.32143) -- (-0.29269, -0.35017) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](-0.39286, -0.39286) -- (-0.35237, -0.3964) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](-0.094156, -0.3949) -- (-0.040644, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, -0.28571) -- (-0.25, -0.25) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.2, -0.5) -- (-0.22613, -0.46887) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.1, -0.45936) -- (-0.094156, -0.3949) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](-0.22613, -0.46887) -- (-0.25, -0.5) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.17613) -- (-0.040644, -0.15) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](-0.2449, -0.40584) -- (-0.28094, -0.32497) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](-0.040644, -0.45) -- (0, -0.45) -- (0, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.05) -- (0, -0.1) -- (-0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0, -0.3) -- (-0.031135, -0.27613) -- (0, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](-0.040644, -0.35) -- (-0.094156, -0.2949) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](-0.040644, -0.35) -- (0, -0.3) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](-0.2, -0.3895) -- (-0.22126, -0.27874) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](-0.031135, -0.27613) -- (0, -0.3) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](-0.040644, -0.45) -- (-0.031135, -0.37613) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](-0.040644, -0.35) -- (0, -0.35) -- (-0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](-0.040644, -0.25) -- (-0.031135, -0.27613) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](-0.040644, -0.25) -- (0, -0.25) -- (-0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0, -0.2) -- (-0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](-0.040644, -0.25) -- (-0.031135, -0.17613) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](-0.040644, -0.25) -- (-0.094156, -0.2949) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.031135, -0.076125) -- (-0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.10714, -0.10714) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.040644, -0.15) -- (-0.031135, -0.17613) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](-0.17857, -0.17857) -- (-0.13808, -0.18211) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.040644, -0.15) -- (-0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.13808, -0.18211) -- (-0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](-0.22126, -0.27874) -- (-0.20951, -0.25354) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.13808, -0.18211) -- (-0.040644, -0.25) -- (-0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.13808, -0.18211) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.14983, -0.20731) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.20951, -0.25354) -- (-0.14983, -0.20731) -- (-0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, -0.28571) -- (-0.28094, -0.32497) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](-0.32143, -0.32143) -- (-0.28094, -0.32497) -- (-0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](-0.094156, -0.3949) -- (-0.094156, -0.2949) -- (-0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.28571, -0.28571) -- (-0.22126, -0.27874) -- (-0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.25, -0.25) -- (-0.21429, -0.21429) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](-0.15, -0.5) -- (-0.2, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](-0.28094, -0.32497) -- (-0.22126, -0.27874) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](-0.25, -0.25) -- (-0.20951, -0.25354) -- (-0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.21429, -0.21429) -- (-0.14983, -0.20731) -- (-0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.32613, -0.46887) -- (-0.3, -0.45936) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](-0.2449, -0.40584) -- (-0.2, -0.3895) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](-0.36412, -0.4216) -- (-0.35237, -0.3964) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](-0.35714, -0.35714) -- (-0.29269, -0.35017) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](-0.4, -0.45936) -- (-0.36412, -0.4216) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](-0.39286, -0.39286) -- (-0.35714, -0.35714) -- (-0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](-0.4, -0.45936) -- (-0.42857, -0.42857) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](-0.4, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](-0.42857, -0.42857) -- (-0.39286, -0.39286) -- (-0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](-0.42613, -0.46887) -- (-0.42857, -0.42857) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](-0.42613, -0.46887) -- (-0.46429, -0.46429) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.5, -0.5) -- (-0.46429, -0.46429) -- (-0.45, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](-0.35, -0.5) -- (-0.4, -0.5) -- (-0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.45, -0.5) -- (-0.46429, -0.46429) -- (-0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](-0.45, -0.5) -- (-0.42613, -0.46887) -- (-0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](-0.4, -0.45936) -- (-0.32613, -0.46887) -- (-0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](-0.36412, -0.4216) -- (-0.3, -0.45936) -- (-0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](-0.35, -0.5) -- (-0.32613, -0.46887) -- (-0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](-0.12613, -0.46887) -- (-0.1, -0.5) -- (-0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](-0.22613, -0.46887) -- (-0.3, -0.45936) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](-0.3, -0.5) -- (-0.3, -0.45936) -- (-0.25, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](-0.2, -0.45936) -- (-0.22613, -0.46887) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](-0.2, -0.5) -- (-0.25, -0.5) -- (-0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.12613, -0.46887) -- (-0.2, -0.45936) -- (-0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](-0.12613, -0.46887) -- (-0.15, -0.5) -- (-0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](-0.35237, -0.3964) -- (-0.2449, -0.40584) -- (-0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](-0.29269, -0.35017) -- (-0.28094, -0.32497) -- (-0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](-0.2, -0.3895) -- (-0.094156, -0.3949) -- (-0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](-0.2, -0.3895) -- (-0.094156, -0.2949) -- (-0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](-0.040644, -0.45) -- (0, -0.4) -- (0, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](-0.031135, -0.37613) -- (0, -0.35) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](-0.12613, -0.46887) -- (-0.1, -0.45936) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](-0.094156, -0.3949) -- (-0.031135, -0.37613) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](-0.05, -0.5) -- (-0.1, -0.45936) -- (-0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](-0.12613, -0.46887) -- (-0.094156, -0.3949) -- (-0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](-0.1, -0.45936) -- (-0.05, -0.5) -- (-0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](-0.040644, -0.45) -- (0, -0.5) -- (-0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.40584, -0.2449) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](-0.32143, -0.32143) -- (-0.35017, -0.29269) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, -0.22126) -- (-0.28571, -0.28571) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.5, -0.1) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.40584, -0.2449) -- (-0.35017, -0.29269) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3964, -0.35237) -- (-0.35017, -0.29269) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.8555; green,51.2805; blue,205.0965},draw={rgb,255: red,67.8555; green,51.2805; blue,205.0965}](-0.39286, -0.39286) -- (-0.3964, -0.35237) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, -0.094156) -- (-0.3895, -0.2) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](-0.32497, -0.28094) -- (-0.35017, -0.29269) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0) -- (-0.4, 0) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3895, -0.2) -- (-0.40584, -0.2449) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.37613, -0.031135) -- (-0.3949, -0.094156) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27613, -0.031135) -- (-0.35, -0.040644) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.20731, -0.14983) -- (-0.25354, -0.20951) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.2, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.035714, -0.035714) -- (-0.076125, -0.031135) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.15, -0.040644) -- (-0.076125, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.076125, -0.031135) -- (-0.15, -0.040644) -- (-0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.1, 0) -- (-0.076125, -0.031135) -- (-0.05, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2949, -0.094156) -- (-0.20731, -0.14983) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](-0.28571, -0.28571) -- (-0.32497, -0.28094) -- (-0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](-0.21429, -0.21429) -- (-0.25354, -0.20951) -- (-0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, -0.094156) -- (-0.46887, -0.12613) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, -0.13808) -- (-0.15, -0.040644) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.20731, -0.14983) -- (-0.21429, -0.21429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, -0.22126) -- (-0.25, -0.25) -- (-0.25354, -0.20951) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25354, -0.20951) -- (-0.2949, -0.094156) -- (-0.27874, -0.22126) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.15) -- (-0.5, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.25) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.311; green,43.0695; blue,183.0645},draw={rgb,255: red,64.311; green,43.0695; blue,183.0645}](-0.3964, -0.35237) -- (-0.35714, -0.35714) -- (-0.35017, -0.29269) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.014; green,49.266; blue,199.614},draw={rgb,255: red,67.014; green,49.266; blue,199.614}](-0.27874, -0.22126) -- (-0.32497, -0.28094) -- (-0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27874, -0.22126) -- (-0.3895, -0.2) -- (-0.32497, -0.28094) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.5, -0.3) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.40584, -0.2449) -- (-0.45936, -0.3) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.329; green,60.741; blue,223.5585},draw={rgb,255: red,70.329; green,60.741; blue,223.5585}](-0.3964, -0.35237) -- (-0.39286, -0.39286) -- (-0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, -0.36412) -- (-0.42857, -0.42857) -- (-0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, -0.36412) -- (-0.46887, -0.32613) -- (-0.45936, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4216, -0.36412) -- (-0.45936, -0.4) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.45) -- (-0.5, -0.5) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.46887, -0.42613) -- (-0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.42613) -- (-0.5, -0.45) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.42857, -0.42857) -- (-0.46887, -0.42613) -- (-0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.35) -- (-0.5, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.4) -- (-0.5, -0.45) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.4) -- (-0.5, -0.4) -- (-0.46887, -0.42613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.46887, -0.32613) -- (-0.4216, -0.36412) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.3) -- (-0.4216, -0.36412) -- (-0.3964, -0.35237) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.46887, -0.22613) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.2) -- (-0.5, -0.25) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.46887, -0.32613) -- (-0.5, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.35) -- (-0.45936, -0.4) -- (-0.46887, -0.32613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.45936, -0.3) -- (-0.40584, -0.2449) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.22613) -- (-0.5, -0.25) -- (-0.45936, -0.3) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.45936, -0.2) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.5, -0.15) -- (-0.45936, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27874, -0.22126) -- (-0.2949, -0.094156) -- (-0.3895, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3949, -0.094156) -- (-0.37613, -0.031135) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.27613, -0.031135) -- (-0.2949, -0.094156) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, -0.040644) -- (-0.3949, -0.094156) -- (-0.2949, -0.094156) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45936, -0.1) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.46887, -0.12613) -- (-0.3949, -0.094156) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.1) -- (-0.46887, -0.12613) -- (-0.45936, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.2) -- (-0.5, -0.2) -- (-0.46887, -0.22613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.15) -- (-0.46887, -0.12613) -- (-0.5, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, 0) -- (-0.45, -0.040644) -- (-0.45, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45936, -0.1) -- (-0.3949, -0.094156) -- (-0.45, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.45, 0) -- (-0.45, -0.040644) -- (-0.4, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.5, -0.05) -- (-0.45, -0.040644) -- (-0.5, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.35, 0) -- (-0.37613, -0.031135) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.4, 0) -- (-0.45, -0.040644) -- (-0.37613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0) -- (-0.35, 0) -- (-0.35, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0) -- (-0.3, 0) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2, 0) -- (-0.25, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17613, -0.031135) -- (-0.2, 0) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, 0) -- (-0.27613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.3, 0) -- (-0.35, -0.040644) -- (-0.27613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.17857, -0.17857) -- (-0.18211, -0.13808) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.10714, -0.10714) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.14286, -0.14286) -- (-0.18211, -0.13808) -- (-0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.25, -0.040644) -- (-0.20731, -0.14983) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.2949, -0.094156) -- (-0.25354, -0.20951) -- (-0.20731, -0.14983) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.10714, -0.10714) -- (-0.15, -0.040644) -- (-0.18211, -0.13808) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.071429, -0.071429) -- (-0.15, -0.040644) -- (-0.10714, -0.10714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.076125, -0.031135) -- (-0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.18211, -0.13808) -- (-0.17613, -0.031135) -- (-0.25, -0.040644) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, -0.040644) -- (-0.15, 0) -- (-0.17613, -0.031135) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.15, 0) -- (-0.15, -0.040644) -- (-0.1, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](-0.05, 0) -- (-0.035714, -0.035714) -- (0, 0) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.349; green,87.2355; blue,247.401},draw={rgb,255: red,71.349; green,87.2355; blue,247.401}](0.35237, -0.3964) -- (0.35714, -0.35714) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.071429, -0.071429) -- (0.035714, -0.035714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.359; green,131.019; blue,249.033},draw={rgb,255: red,46.359; green,131.019; blue,249.033}](0.36412, -0.4216) -- (0.35237, -0.3964) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.6725; green,231.642; blue,36.975},draw={rgb,255: red,244.6725; green,231.642; blue,36.975}](0.1, -0.5) -- (0.1, -0.45936) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,250.0785; green,212.721; blue,45.5685},draw={rgb,255: red,250.0785; green,212.721; blue,45.5685}](0.2, -0.5) -- (0.2, -0.45936) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.076125) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.2) -- (0.031135, -0.17613) -- (0, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,42.0495; green,146.7525; blue,237.7365},draw={rgb,255: red,42.0495; green,146.7525; blue,237.7365}](0.094156, -0.2949) -- (0.040644, -0.35) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.1) -- (0.031135, -0.076125) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.5785; green,84.4815; blue,245.718},draw={rgb,255: red,71.5785; green,84.4815; blue,245.718}](0.14983, -0.20731) -- (0.040644, -0.25) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.5805; green,48.2715; blue,196.8345},draw={rgb,255: red,66.5805; green,48.2715; blue,196.8345}](0.031135, -0.17613) -- (0.040644, -0.25) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.6595; green,126.8625; blue,251.022},draw={rgb,255: red,47.6595; green,126.8625; blue,251.022}](0.040644, -0.35) -- (0.094156, -0.2949) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.2, -0.3895) -- (0.094156, -0.3949) -- (0.12613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.040644, -0.45) -- (0.094156, -0.3949) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.085; green,101.3115; blue,253.062},draw={rgb,255: red,68.085; green,101.3115; blue,253.062}](0.22126, -0.27874) -- (0.2, -0.3895) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.071429, -0.071429) -- (0.031135, -0.076125) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.39286, -0.39286) -- (0.35714, -0.35714) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0195; green,202.3935; blue,139.077},draw={rgb,255: red,66.0195; green,202.3935; blue,139.077}](0.4, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.45, -0.5) -- (0.5, -0.5) -- (0.46429, -0.46429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.45, -0.5) -- (0.46429, -0.46429) -- (0.42613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,93.6105; green,204.5355; blue,116.3565},draw={rgb,255: red,93.6105; green,204.5355; blue,116.3565}](0.4, -0.5) -- (0.4, -0.45936) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.094; green,66.249; blue,230.3925},draw={rgb,255: red,71.094; green,66.249; blue,230.3925}](0.42613, -0.46887) -- (0.46429, -0.46429) -- (0.42857, -0.42857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.4765; green,85.8585; blue,246.585},draw={rgb,255: red,71.4765; green,85.8585; blue,246.585}](0.42613, -0.46887) -- (0.42857, -0.42857) -- (0.4, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,46.053; green,132.3705; blue,248.319},draw={rgb,255: red,46.053; green,132.3705; blue,248.319}](0.4, -0.45936) -- (0.36412, -0.4216) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,83.1045; blue,244.8},draw={rgb,255: red,71.6295; green,83.1045; blue,244.8}](0.4, -0.45936) -- (0.42857, -0.42857) -- (0.36412, -0.4216) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.32613, -0.46887) -- (0.3, -0.45936) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0.22613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.2449, -0.40584) -- (0.35237, -0.3964) -- (0.29269, -0.35017) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,74.715; blue,238.476},draw={rgb,255: red,71.6805; green,74.715; blue,238.476}](0.36412, -0.4216) -- (0.42857, -0.42857) -- (0.39286, -0.39286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,180.8205; green,197.0385; blue,50.949},draw={rgb,255: red,180.8205; green,197.0385; blue,50.949}](0.4, -0.45936) -- (0.32613, -0.46887) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,21.8025; green,175.0575; blue,217.0815},draw={rgb,255: red,21.8025; green,175.0575; blue,217.0815}](0.36412, -0.4216) -- (0.3, -0.45936) -- (0.32613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,229.5; green,187.068; blue,44.5995},draw={rgb,255: red,229.5; green,187.068; blue,44.5995}](0.32613, -0.46887) -- (0.3, -0.5) -- (0.35, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,54.009; green,199.614; blue,152.5665},draw={rgb,255: red,54.009; green,199.614; blue,152.5665}](0.45, -0.5) -- (0.42613, -0.46887) -- (0.4, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,238.6035; green,185.895; blue,52.5555},draw={rgb,255: red,238.6035; green,185.895; blue,52.5555}](0.3, -0.45936) -- (0.25, -0.5) -- (0.3, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.553; green,71.8845; blue,236.0025},draw={rgb,255: red,71.553; green,71.8845; blue,236.0025}](0.32143, -0.32143) -- (0.29269, -0.35017) -- (0.35714, -0.35714) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,253.9035; green,200.328; blue,52.3515},draw={rgb,255: red,253.9035; green,200.328; blue,52.3515}](0.25, -0.5) -- (0.3, -0.45936) -- (0.22613, -0.46887) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.86; green,217.4895; blue,43.2225},draw={rgb,255: red,247.86; green,217.4895; blue,43.2225}](0.25, -0.5) -- (0.22613, -0.46887) -- (0.2, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,40.1115; green,149.277; blue,235.977},draw={rgb,255: red,40.1115; green,149.277; blue,235.977}](0.3, -0.45936) -- (0.35237, -0.3964) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,249.1095; green,250.8945; blue,20.5275},draw={rgb,255: red,249.1095; green,250.8945; blue,20.5275}](0.12613, -0.46887) -- (0.1, -0.5) -- (0.15, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,244.7235; green,233.1465; blue,36.159},draw={rgb,255: red,244.7235; green,233.1465; blue,36.159}](0.12613, -0.46887) -- (0.1, -0.45936) -- (0.1, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,247.197; green,219.0705; blue,42.4575},draw={rgb,255: red,247.197; green,219.0705; blue,42.4575}](0.040644, -0.45) -- (0, -0.5) -- (0.05, -0.5) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,19.635; green,190.434; blue,184.212},draw={rgb,255: red,19.635; green,190.434; blue,184.212}](0.1, -0.45936) -- (0.12613, -0.46887) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,47.2515; green,196.8855; blue,162.6645},draw={rgb,255: red,47.2515; green,196.8855; blue,162.6645}](0, -0.45) -- (0.040644, -0.45) -- (0, -0.4) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,251.4555; green,209.559; blue,47.073},draw={rgb,255: red,251.4555; green,209.559; blue,47.073}](0, -0.45) -- (0, -0.5) -- (0.040644, -0.45) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,27.6675; green,170.0595; blue,222.717},draw={rgb,255: red,27.6675; green,170.0595; blue,222.717}](0.031135, -0.37613) -- (0.094156, -0.3949) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,5.967; green,181.1265; blue,207.162},draw={rgb,255: red,5.967; green,181.1265; blue,207.162}](0.2449, -0.40584) -- (0.22613, -0.46887) -- (0.3, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,26.0865; green,191.505; blue,180.744},draw={rgb,255: red,26.0865; green,191.505; blue,180.744}](0.040644, -0.45) -- (0.1, -0.45936) -- (0.094156, -0.3949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,246.6105; green,220.677; blue,41.718},draw={rgb,255: red,246.6105; green,220.677; blue,41.718}](0.040644, -0.45) -- (0.05, -0.5) -- (0.1, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.459; green,185.5125; blue,197.676},draw={rgb,255: red,0.459; green,185.5125; blue,197.676}](0.12613, -0.46887) -- (0.2, -0.45936) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,245.259; green,237.66; blue,33.252},draw={rgb,255: red,245.259; green,237.66; blue,33.252}](0.12613, -0.46887) -- (0.15, -0.5) -- (0.2, -0.45936) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,3.9525; green,181.8915; blue,205.632},draw={rgb,255: red,3.9525; green,181.8915; blue,205.632}](0.2, -0.45936) -- (0.2449, -0.40584) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,22.9245; green,190.9695; blue,182.478},draw={rgb,255: red,22.9245; green,190.9695; blue,182.478}](0.2, -0.45936) -- (0.22613, -0.46887) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,25.7295; green,172.125; blue,220.6515},draw={rgb,255: red,25.7295; green,172.125; blue,220.6515}](0, -0.35) -- (0.031135, -0.37613) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,0.4845; green,184.11; blue,200.889},draw={rgb,255: red,0.4845; green,184.11; blue,200.889}](0, -0.4) -- (0.040644, -0.45) -- (0.031135, -0.37613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,68.952; green,54.519; blue,212.823},draw={rgb,255: red,68.952; green,54.519; blue,212.823}](0.21429, -0.21429) -- (0.14983, -0.20731) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.812; green,111.639; blue,254.7705},draw={rgb,255: red,61.812; green,111.639; blue,254.7705}](0.040644, -0.25) -- (0.031135, -0.27613) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,58.9305; green,114.6735; blue,254.8725},draw={rgb,255: red,58.9305; green,114.6735; blue,254.8725}](0, -0.25) -- (0.031135, -0.27613) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.5175; green,135.048; blue,246.7635},draw={rgb,255: red,45.5175; green,135.048; blue,246.7635}](0, -0.3) -- (0, -0.35) -- (0.040644, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,49.725; green,123.9555; blue,252.1185},draw={rgb,255: red,49.725; green,123.9555; blue,252.1185}](0, -0.3) -- (0.040644, -0.35) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,23.307; green,174.114; blue,218.331},draw={rgb,255: red,23.307; green,174.114; blue,218.331}](0, -0.4) -- (0.031135, -0.37613) -- (0, -0.35) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.178; green,107.1765; blue,254.1075},draw={rgb,255: red,65.178; green,107.1765; blue,254.1075}](0, -0.25) -- (0, -0.3) -- (0.031135, -0.27613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.035714, -0.035714) -- (0, 0) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.040644, -0.15) -- (0, -0.1) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0, -0.25) -- (0.040644, -0.25) -- (0, -0.2) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0, -0.15) -- (0.031135, -0.17613) -- (0.040644, -0.15) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.688; green,46.257; blue,191.2755},draw={rgb,255: red,65.688; green,46.257; blue,191.2755}](0, -0.2) -- (0.040644, -0.25) -- (0.031135, -0.17613) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.031135, -0.076125) -- (0.035714, -0.035714) -- (0, -0.05) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.10714, -0.10714) -- (0.071429, -0.071429) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.040644, -0.15) -- (0.031135, -0.17613) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,65.229; green,45.2115; blue,188.5215},draw={rgb,255: red,65.229; green,45.2115; blue,188.5215}](0.14983, -0.20731) -- (0.13808, -0.18211) -- (0.040644, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.040644, -0.15) -- (0.13808, -0.18211) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.10714, -0.10714) -- (0.13808, -0.18211) -- (0.14286, -0.14286) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.14286, -0.14286) -- (0.13808, -0.18211) -- (0.17857, -0.17857) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,60.4095; green,113.1435; blue,254.898},draw={rgb,255: red,60.4095; green,113.1435; blue,254.898}](0.2, -0.3895) -- (0.22126, -0.27874) -- (0.094156, -0.2949) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,64.77; green,44.166; blue,185.793},draw={rgb,255: red,64.77; green,44.166; blue,185.793}](0.17857, -0.17857) -- (0.13808, -0.18211) -- (0.14983, -0.20731) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,57.375; green,116.2545; blue,254.6175},draw={rgb,255: red,57.375; green,116.2545; blue,254.6175}](0.29269, -0.35017) -- (0.28094, -0.32497) -- (0.2449, -0.40584) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,43.758; green,144.2025; blue,239.5215},draw={rgb,255: red,43.758; green,144.2025; blue,239.5215}](0.094156, -0.2949) -- (0.094156, -0.3949) -- (0.2, -0.3895) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.757; green,77.52; blue,240.7455},draw={rgb,255: red,71.757; green,77.52; blue,240.7455}](0.25, -0.25) -- (0.20951, -0.25354) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.14983, -0.20731) -- (0.094156, -0.2949) -- (0.20951, -0.25354) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,66.0705; green,105.6975; blue,253.8525},draw={rgb,255: red,66.0705; green,105.6975; blue,253.8525}](0.36412, -0.4216) -- (0.39286, -0.39286) -- (0.35237, -0.3964) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.25, -0.25) -- (0.22126, -0.27874) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,45.7725; green,133.722; blue,247.5795},draw={rgb,255: red,45.7725; green,133.722; blue,247.5795}](0.2, -0.3895) -- (0.2449, -0.40584) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,70.533; green,62.0925; blue,225.42},draw={rgb,255: red,70.533; green,62.0925; blue,225.42}](0.28094, -0.32497) -- (0.32143, -0.32143) -- (0.28571, -0.28571) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,69.513; green,97.002; blue,251.9655},draw={rgb,255: red,69.513; green,97.002; blue,251.9655}](0.28094, -0.32497) -- (0.29269, -0.35017) -- (0.32143, -0.32143) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6295; green,73.3125; blue,237.2775},draw={rgb,255: red,71.6295; green,73.3125; blue,237.2775}](0.28571, -0.28571) -- (0.22126, -0.27874) -- (0.28094, -0.32497) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,71.6805; green,81.702; blue,243.8565},draw={rgb,255: red,71.6805; green,81.702; blue,243.8565}](0.20951, -0.25354) -- (0.094156, -0.2949) -- (0.22126, -0.27874) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,67.4475; green,50.286; blue,202.3935},draw={rgb,255: red,67.4475; green,50.286; blue,202.3935}](0.21429, -0.21429) -- (0.20951, -0.25354) -- (0.25, -0.25) -- cycle;
\path[line cap=round,line width=0.01mm,fill={rgb,255: red,61.761; green,38.352; blue,168.3765},draw={rgb,255: red,61.761; green,38.352; blue,168.3765}](0.17857, -0.17857) -- (0.14983, -0.20731) -- (0.21429, -0.21429) -- cycle;


==> images/twoLongDipoles.tex <==
\draw[draw=none,fill=mycolor] (-0.00600000, -0.12741179) -- (0.00600000, -0.12741179) -- (0.00600000, 0.12741179) -- (-0.00600000, 0.12741179) -- cycle;
\draw[draw=none,fill=mycolor] (-0.00600000, 0.14240142) -- (0.00600000, 0.14240142) -- (0.00600000, 0.39722501) -- (-0.00600000, 0.39722501) -- cycle;

